Novel constraints on fermionic dark matter from galactic observables II: galaxy scaling relations

We have recently introduced in paper I an extension of the Ruffini-Arg\"uelles-Rueda (RAR) model for the distribution of DM in galaxies, by including for escape of particle effects. Being built upon self-gravitating fermions at finite temperatures, the RAR solutions develop a characteristic \textit{dense quantum core-diluted halo} morphology which, for fermion masses in the range $mc^2 \approx 10-345$ keV, was shown to provide good fits to the Milky Way rotation curve. We study here for the first time the applicability of the extended RAR model to other structures from dwarfs to ellipticals to galaxy clusters, pointing out the relevant case of $mc^2 = 48$ keV. By making a full coverage of the remaining free parameters of the theory, and for each galactic structure, we present a complete family of astrophysical RAR profiles which satisfy realistic halo boundary conditions inferred from observations. Each family-set of RAR solutions predicts given windows of total halo masses and central quantum-core masses, the latter opening the interesting possibility to interpret them as alternatives either to intermediate-mass BHs (for dwarf galaxies), or to supermassive BHs (SMBHs, in the case of larger galaxy types). The model is shown to be in good agreement with different observationally inferred scaling relations such as: (1) the Ferrarese relation connecting DM halos with supermassive dark central objects; and (2) the nearly constant DM surface density of galaxies. Finally, the theory provides a natural mechanism for the formation of SMBHs of few $10^8 M_\odot$ via the gravitational collapse of unstable DM quantum-cores.

==> content/introduction-OLD.tex <==
\section{Introduction}
\label{sec:introduction}
The problem of describing \ac{DM} halos in terms of fundamental particles has gained considerable attention in the last years, given they may provide solutions to many of the unsuccessful predictions of the \ac{CDM} paradigm arising below $\sim\SI{10}{\kilo\parsec}$ scales. The majority of such models are comprised within the following three different approaches:
(i) The case of ultra light bosons with masses in the range $m_bc^2\sim \SIrange{1}{100E-22}{\eV}$, known as ultra light \ac{DM}, \ac{FDM} or scalar field \ac{DM} \citep{1983PhLB..122..221B,1994PhRvD..50.3650S,2000PhRvL..85.1158H,2001PhRvD..63f3506M,2012MNRAS.422..282R,2017PhRvD..95d3541H,2018arXiv180500122B};
(ii) the case of Thomas-Fermi models based on fully-degenerate fermions with masses $m_{df}c^2\sim$ few $\SI{E2}{\eV}$ \citep{2013NewA...22...39D,2015JCAP...01..002D,2017MNRAS.467.1515R}.  We also include in this group similar models based on self-gravitating fermions but in the dilute regime (i.e. Boltzmannian-like) which, however, \textit{do not} imply an explicit particle mass dependence when contrasted with halo observables \citep[see e.g.][]{2014MNRAS.442.2717D};
(iii) the \ac{RAR} model based on semi-degenerate configurations of self-gravitating fermions accounting for finite temperature and for relativistic effects, with masses in the range $m_fc^2\sim$ few $\SIrange{E1}{E2}{\kilo\eV}$ \citep{2013pdmg.conf30204A,2014IJMPD..2342020A,2015MNRAS.451..622R,2015ARep...59..656S,2016JCAP...04..038A,2016PhRvD..94l3004G,2018PDU....21...82A}.

One of the main interesting aspects of the above models is the particle mass dependence on their density profiles (besides the other physically-motivated free parameters), differently to the case of phenomenological profiles existing in the literature aiming to fit results from classical N-body numerical simulations. Moreover, such kind of self-gravitating systems of particles opens the possibility to have direct access to the nature, mass, and explicit phase-space distributions dependence at the onset of halo formation (see e.g., ~\citealp{2017PhRvD..95d3541H} and refs. therein, for the case of bosons and, e.g.~\citealp{2018PDU....21...82A} and refs. therein, for the case of fermions). 

However, not all of the above particle-motivated \ac{DM} halo models have the required cosmological and astrophysical properties when contrasted with different observational data-sets. Some fundamental problems remain mainly within the cases (i) and (ii) such as: (a) galaxy-scaling relations; (b) Ly$\alpha$ forest constraints; (c) nearby disk galaxies with high resolution rotation curve features. 

Concerning the first point (a), we could mention the recent results in \citet{2018PhRvD..98b3513D} which demonstrated that standard \ac{FDM} models without self-interactions\footnote{Composed, for example, by axion-like particles with $m_bc^2\sim\SI{E-22}{\eV}$ as the one proposed in \citet{2000PhRvL..85.1158H,2017PhRvD..95d3541H}.} are ruled out when asking to follow the \ac{DM}-surface-density Universal relation \citep{2009MNRAS.397.1169D,2017MNRAS.470.2410R}. That is, while this observational relation imposes that the central \ac{DM} halo density $\rho_c$ scales with the inverse of the core radius $r_c$ to some power $\beta\approx 1$ (i.e. $\rho_c\sim r_c^{-1}$); the \ac{FDM} theory yields an inverse proportionality relation but with a quite different power $\beta_{\rm FDM}=4$.\footnote{Alternative \ac{FDM} models including for quartic-like self-interactions were also ruled out when contrasted against the above observed \ac{DM} halo Universal-relation in \citet{2018PhRvD..98b3513D}; see however \citet{2012MNRAS.422..282R} for other kind of self-interacting bosons.}

On a different observational ground, and moving to the issue (b), the \ac{DM} particle mass constraints arising from recent Ly$\alpha$ forest observations, put severe bounds both to \ac{FDM} particles (i), as well as to fermions (ii)-(iii). The key concept to understand how all such bounds arise is to recognize that the Ly$\alpha$ forest can be explained in terms of the standard cosmological model \citep[see e.g.][]{1994ApJ...437L...9C}, and therefore it can be directly linked to the matter power spectrum by offering a complementary probe for it~\citep{1999ApJ...516..519H}. 

Regarding (i), \ac{FDM} has an associated matter power spectrum which share the same features with the one of the \ac{WDM} paradigm at large scales, both exhibiting a clear drop (though somewhat different in shape) in power below a given scale~\citep{2014MNRAS.437.2652M}. Such similar behaviour allowed \citet{2017PhRvD..95d3541H} to roughly relate the lower bound mass values of \ac{FDM} to the ones of a \ac{WDM} fermion obtained by \citet{{2013PhRvD..88d3502V}} from Ly$\alpha$ forest data. In particular, a lower limit of $\SI{2.5}{\kilo\eVcc}$ (at $3-\sigma$) of the hypothetical \ac{WDM} particle (thermal relics) translates into $m_bc^2 > \SI{E-21}{\eV}$ for the ultra light boson at the same confidence level \citep{2017PhRvD..95d3541H}. Unfortunately, this bound strongly disfavours the typical \ac{FDM} range of masses needed to solve different small-scale issues of the CDM paradigm \citep{2017PhRvD..95d3541H}. Improved analysis making use of dedicated cosmological simulations within \ac{FDM} paradigm to account for the physics at the scales probed by the Ly$\alpha$ forest data (from the BOSS survey), exclude the mass range $m_b = \SIrange{E-22}{2.3E-21}{\eV}$ \citep{2017MNRAS.471.4606A}. 

In the case of fermionic models, it is then clear that the $\sim$ few \si{\kilo\eV} lower bound found in \citet[][see also~\citet{2017JCAP...06..047Y} for more general lower bounds above \si{\kilo\eV} including for sterile neutrino \ac{WDM}]{2013PhRvD..88d3502V} is in  tension with the below-\si{\kilo\eV} Thomas-Fermi models cited above in (ii), while it remains in agreement with the \ac{RAR} model introduced in (iii).

Reproducing the (total) Milky Way rotation curve features mentioned in (c) posses as well serious challenges to \ac{FDM} models (i) in the desired mass range needed to account for other astrophysical and small-scale cosmological observables \citep{2018arXiv180500122B}. Indeed, it was there explicitly shown that the solitonic core arising typically at bulge-scales in the case of typical disk galaxies as the ones there analyzed, practically excludes the \ac{FDM} mass range $m_b = \SIrange{E-22}{E-21}{\eV}$. Finally, the case for highly degenerate fermionic halos as introduced in (ii), are not applicable at all to reproduce the rotation curves of disk galaxies (or larger), since they were originally motivated to fit the dispersion velocities of small dSphs \citep{2013NewA...22...39D} due to the predicted highly compact and small sized halos. Moreover, a closer look implies that Thomas-Fermi models as the ones recently analyzed in~\citet{2015JCAP...01..002D} are disfavoured even to fit dSph dispersion velocities, and the artificial introduction of an isothermal tail is needed \citep{2017MNRAS.467.1515R}.

We will show that the results of this work, together with the ones of the first article of this series~\citep[][hereafter Paper I]{2018PDU....21...82A} on the fit to the Milky Way full rotation curve (together with other disc galaxy fittings), and the discussion of the constraints put to \acs{LCDM} and \acs{LWDM} cosmologies by the Ly$\alpha$ forest, favour instead the $\si{\kilo\eV}$ fermionic \ac{RAR} model (iii).

In \cref{sec:other:results} we present the application of the extended \ac{RAR} theory to different galaxy types, and for fermion masses in the range limited by the Milky Way constraints. A more detailed description of the obtained families focusing on the configuration parameters is given in \cref{sec:application:other:analysis}. We also briefly compare in \cref{sec:robustness} the applied method with an alternative set of constraints for dwarfs to verify its robustness.

Further, we demonstrate in \cref{sec:application:other:correlations} that the results of our model are consistent with (a) the observationally inferred correlations between the mass of the dark central object and total \ac{DM} halo mass \citep{2002ApJ...578...90F,2011Natur.469..377K,2015ApJ...800..124B}, and with (b) the observationally inferred (universal) value of the inner surface density of \ac{DM} halos \citep{2009MNRAS.397.1169D}, from dwarf to elliptical galaxies.

Finally, in \cref{sec:conclusion} we summarize the conclusions of our results.

==> figures/ferrarese/figure.tex <==
\begin{figure*}[t!]%
	\centering%
	\includegraphics[width=0.8\hsize]{\ROOTPATH/fig.pdf}
	\caption{Prediction of the $\Mcore$-$\Mtot$ relations within three parametric \ac{RAR} model (for $mc^2 = \SI{48}{\kilo\eV}$). The different \textit{predicted} lines read for each galaxy type in correspondence with the astrophysical \ac{RAR} solutions as given in \cref{fig:profiles}. The results show the ability to be in agreement with the different $\MBH-\Mtot$ relations, as considered in the literature, and explicited in this picture box. The filled-black dots correspond to the critical core masses $\McoreCR$, and the empty-black dot indicates the limiting maximum core mass for dwarfs $\McoreMAX$.}%
	\label{fig:McMDM}%
\end{figure*}
